Top Quark Physics

We review the prospects for studies of the top quark at the LHC.

==> rlfig.tex <==
% pomiedzy \makeatletter i \makeatother mozna wkopiowac swoj .sty
\makeatletter
%   26/10/88 810261839  MEMBER NAME  ZLRF     (PHD)      M  TEX
%   23/09/87 709231736	MEMBER NAME  LRF	    (IMPL)	 M  TEX		
% Macros for right and left side figures
%   MGH  7/7/86  initial coding
% modified for easy use with LaTeX by p.k.schilling desy
% modified for allowing user interference Z. Jakubowski desy		
% Arguments:
    %[#1]- number of lines to be added or subtracted from picture space 	
    % #2 - box to cover figure space
    % #3 - figure caption text
%
% Usage: e.g.
    % \rightfig{\begin{picture}(width,height)\end{picture}}
    %                                {This is the caption}%
    % The '%' at the end of \rightfig is needed to keep extra space out
    % Use \hangover after each paragraph that might have the figure
    % beside it
% side figure macros' variables
    \newdimen\figwidth     % figure box width
    \newdimen\boxht        % figure box height
    \newdimen\boxwd        % figure box width
    \newbox\figbox         % figure box
    \newbox\capbox         % caption box, used for caption indent
    \newbox\dumybox        % used for font height
    \newdimen\lineht       % font height dimension
    \newcount\nlines       % number of lines to hang indent text beside figure
    \newcount\linehtint    % font height integer sp's, scaled points
%
% rightfig - Leaves space for right column figure with caption
\def\rightfig{\@ifnextchar [{\@rightfig}{\@rightfig[0]}}%
\def\@rightfig[#1]#2#3{%
\refstepcounter{figure}%
    \figwidth=\hsize%             % save current hsize
    \setbox\capbox = \hbox{\fnum@figure:\ }%
    \setbox\figbox =\hbox{#2}%:   % setup the figure space
    \boxwd=\wd\figbox%            % save the box height
    \setbox\figbox =\vbox{\hsize\boxwd%
     \hbox{#2}%  % setup the figure space
%    \hangindent=\wd\capbox \hangafter=1%
     \noindent\box\capbox #3}%
    \boxht=\ht\figbox%            % save the box height
    \boxwd=\wd\figbox%            % save the box height
    \advance\figwidth by -\boxwd%
    {\ht\figbox=0pt \moveright\figwidth \box\figbox}% % put the figure in
    \vskip-\parskip \vskip-4.0pt%   %paragraph beside the figure:
    \setbox\dumybox=\vbox{\strut}%  % get the height and depth of a line
    \lineht=\ht\dumybox \advance\lineht by \dp\dumybox%
    \linehtint=\lineht \nlines=\boxht% % scale and truncate dimensions
    \divide\nlines by \linehtint%      % box height/line height = # of lines
    \advance\nlines by 2%   % find par width
    \advance\nlines by #1%
    \figwidth=\boxwd\advance\figwidth by 0.25in%
    \hangindent=-\the\figwidth \hangafter=-\the\nlines%%
}
%
% leftfig - leave space for left column figure with caption, needs
% declarations before rightfig
\def\leftfig{\@ifnextchar [{\@leftfig}{\@leftfig[0]}}%
\def\@leftfig[#1]#2#3{%
\refstepcounter{figure}%
    \figwidth=\hsize%    % save current hsize
    \setbox\capbox = \hbox{\fnum@figure:\ }%
    \setbox\figbox =\hbox{#2}%:   % setup the figure space
    \boxwd=\wd\figbox%    % save the box height
    \setbox\figbox =\vbox{\hsize\boxwd%
  \hbox{#2}% % setup the figure space
%    \hangindent=\wd\capbox \hangafter=1
     \noindent\box\capbox #3}%
    \boxht=\ht\figbox%    % save the box height
    \boxwd=\wd\figbox%    % save the box height
    \advance\figwidth by -\boxwd%
    {\ht\figbox=0pt\box\figbox}% % put the figure in
    \vskip-\parskip \vskip-4.0pt%    %paragraph beside the figure
    \setbox\dumybox=\vbox{\strut}%   % get the height and depth of a line
    \lineht=\ht\dumybox \advance\lineht by \dp\dumybox%
    \linehtint=\lineht \nlines=\boxht%   % scale and truncate dimensions
    \divide\nlines by \linehtint%    % box height/line height = # of lines
    \advance\nlines by 2% % find par width
    \advance\nlines by #1%
    \figwidth=\boxwd\advance\figwidth by 0.25in%
    \hangindent=\the\figwidth \hangafter=-\the\nlines%
}
%
% Continues the hanging indent over between paragrahs, useful for right
% and left figure macros.  It is black magic from the TeXbook p316, ex 14.24
\def\hangover{\edef\next{\hangafter=\the\hangafter
    \hangindent=\the\hangindent}
  \par\next
  \edef\next{\prevgraf=\the\prevgraf}
  \indent\next}
\makeatother

